Thinking Fair and Slow: On the Efficacy of Structured Prompts for Debiasing Language Models

Existing debiasing techniques are typically training-based or require access to the model's internals and output distributions, so they are inaccessible to end-users looking to adapt LLM outputs for their particular needs. In this study, we examine whether structured prompting techniques can offer opportunities for fair text generation. We evaluate a comprehensive end-user-focused iterative framework of debiasing that applies System 2 thinking processes for prompts to induce logical, reflective, and critical text generation, with single, multi-step, instruction, and role-based variants. By systematically evaluating many LLMs across many datasets and different prompting strategies, we show that the more complex System 2-based Implicative Prompts significantly improve over other techniques demonstrating lower mean bias in the outputs with competitive performance on the downstream tasks. Our work offers research directions for the design and the potential of end-user-focused evaluative frameworks for LLM use.

==> checklist.tex <==
A1 Did you discuss the limitations of your work?
A2 Did you discuss any potential risks of your work?
% A3 Do the abstract and introduction summarize the paper’s main claims?
B Did you use or create scientific artifacts?
B1 Did you cite the creators of artifacts you used?
B2 Did you discuss the license or terms for use and/or distribution of any artifacts?
B3 Did you discuss if your use of existing artifact(s) was consistent with their intended use,provided that it was specified? For the artifacts you create, do you specify intended use and whether that is compatible with the original access conditions (in particular, derivatives of data accessed for research purposes should not be used outside of research contexts)?
B4 Did you discuss the steps taken to check whether the data that was collected/used contains any information that names or uniquely identifies individual people or offensive content, and the steps taken to protect / anonymize it?
% B5 Did you provide documentation of the artifacts, e.g., coverage of domains, languages, and linguistic phenomena, demographic groups represented, etc.?
% B6 Did you report relevant statistics like the number of examples, details of train/test/dev splits, etc. for the data that you used/created?
% C Did you run computational experiments?
% C1 Did you report the number of parameters in the models used, the total computational budget (e.g., GPU hours), and computing infrastructure used?
C2 Did you discuss the experimental setup, including hyperparameter search and best-found hyperparameter values?
% C3 Did you report descriptive statistics about your results (e.g., error bars around results,summary statistics from sets of experiments), and is it transparent whether you are reporting the max, mean, etc. or just a single run?
C4 If you used existing packages (e.g., for preprocessing, for normalization, or for evaluation), did you report the implementation, model, and parameter settings used (e.g., NLTK, Spacy, ROUGE, etc.)?
% D Did you use human annotators (e.g., crowdworkers) or research with human subjects?
% D1 Did you report the full text of instructions given to participants, including e.g., screenshots, disclaimers of any risks to participants or annotators, etc.?
% D2 Did you report information about how you recruited (e.g., crowdsourcing platform, students) and paid participants, and discuss if such payment is adequate given the participants’ demographic (e.g., country of residence)?
% D3 Did you discuss whether and how consent was obtained from people whose data you’re using/curating (e.g., did your instructions explain how the data would be used)?
% D4 Was the data collection protocol approved (or determined exempt) by an ethics review board?
% D5 Did you report the basic demographic and geographic characteristics of the annotator population that is the source of the data?




==> crows_table.tex <==
\begin{table}[]
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\multicolumn{1}{l|}{Method}                              & Gender         & Race           & Religion       \\
\midrule
\multicolumn{1}{l|}{GPT2 Medium}                         & 59.16          & 62.4           & 72.38          \\
\multicolumn{1}{l|}{GPT2 Large}                          & 59.16          & 62.21          & 71.43          \\
\multicolumn{1}{l|}{+ Instruction Prefix}                & 51.91          & 61.43          & 73.33          \\
\multicolumn{1}{l|}{+ CoT Prefix}                        & 55.73          & 60.47          & 74.29          \\
\multicolumn{1}{l|}{+ Role Prefix}                       & 55.34          & 62.40           & 72.38          \\
\multicolumn{1}{l|}{+ Fixed Implication}                 & 56.11          & 52.91          & 59.05          \\
\multicolumn{1}{l|}{+ Instruction Implication} & 49.62          & 56.01          & 62.86          \\
\multicolumn{1}{l|}{+ CoT Implication}         & 51.53          & 56.98          & 55.24          \\
\multicolumn{1}{l|}{+ Role Implication}        & 49.24          & 56.20           & 53.33          \\
\multicolumn{1}{l|}{+ Oneshot Implication}               & 50.38          & 56.78          & 53.33          \\
\multicolumn{1}{l|}{+ Few Shot Implication}              & 50.38          & 56.98          & 43.81          \\
\midrule
                                                         &                &                &                \\
\midrule
\multicolumn{1}{l|}{GPTJ}                                & 65.65          & 63.95          & 76.19          \\
\multicolumn{1}{l|}{+ Instruction Prefix}                & 59.16          & 64.92          & 74.29          \\
\multicolumn{1}{l|}{+ CoT Prefix}                        & 63.74          & 68.02          & 79.05          \\
\multicolumn{1}{l|}{+ Role Prefix}                       & 62.6           & 71.32          & 80.00             \\
\multicolumn{1}{l|}{+ Fixed Implication}                 & 51.53          & 54.26          & 48.57          \\
\multicolumn{1}{l|}{+ Instruction Implication} & 52.29          & 50.78          & 47.62          \\
\multicolumn{1}{l|}{+ CoT Implication}         & 51.53          & 51.16          & 45.71          \\
\multicolumn{1}{l|}{+ Role Implication}        & 52.29          & 53.29          & 60.00             \\
\multicolumn{1}{l|}{+ Oneshot Implication}               & \textbf{48.85} & \textbf{49.81} & \textbf{49.52} \\
\multicolumn{1}{l|}{+ Few Shot Implication}              & 54.20           & 52.71          & 53.33          \\
\midrule
                                                         &                &                &                \\
\midrule
\multicolumn{1}{l|}{Pythia}                              & 63.36          & 66.67          & 68.57          \\
\multicolumn{1}{l|}{+ Instruction Prefix}                & 56.11          & 63.95          & 77.14          \\
\multicolumn{1}{l|}{+ CoT Prefix}                        & 60.69          & 66.28          & 73.33          \\
\multicolumn{1}{l|}{+ Role Prefix}                       & 61.45          & 67.25          & 76.19          \\
\multicolumn{1}{l|}{+ Fixed Implication}                 & 50.76          & \textbf{58.14} & 49.52          \\
\multicolumn{1}{l|}{+ Instruction Implication} & \textbf{49.62} & 60.66          & \textbf{48.57} \\
\multicolumn{1}{l|}{+ CoT Implication}         & 50.76          & 59.69          & 55.24          \\
\multicolumn{1}{l|}{+ Role Implication}        & 54.2           & 62.79          & 47.62          \\
\multicolumn{1}{l|}{+ Oneshot Implication}               & 51.53          & 59.88          & \textbf{48.57} \\
\multicolumn{1}{l|}{+ Few Shot Implication}              & 54.58          & 58.14          & 51.43          \\
\midrule
                                                         &                &                &                \\
\midrule
\multicolumn{1}{l|}{Llama 2}                             & 59.54          & 69.96          & 76.19          \\
\multicolumn{1}{l|}{+ Instruction Prefix}                & 57.25          & 70.93          & 83.81          \\
\multicolumn{1}{l|}{+ CoT Prefix}                        & 56.87          & 68.22          & 82.86          \\
\multicolumn{1}{l|}{+ Role Prefix}                       & 58.4           & 69.96          & 85.71          \\
\multicolumn{1}{l|}{+ Fixed Implication}                 & 40.08          & 44.77          & 45.71          \\
\multicolumn{1}{l|}{+ Instruction Implication} & 43.13          & 48.84          & 43.81          \\
\multicolumn{1}{l|}{+ CoT Implication}         & \textbf{46.56} & 46.9           & \textbf{51.43} \\
\multicolumn{1}{l|}{+ Role Implication}        & 42.75          & 50.97          & 45.71          \\
\multicolumn{1}{l|}{+ Oneshot Implication}               & 41.6           & \textbf{49.61} & 44.76          \\
\multicolumn{1}{l|}{+ Few Shot Implication}              & 37.79          & 46.9           & 46.67     \\
\bottomrule
\end{tabular}
}
\end{table}

==> impl_size_abl.tex <==

% \begin{table}
%     \centering
%     \small
%     \begin{tabular}{l|cc}
%     \toprule
% Method&  SS& ICAT \\ \midrule
% Base&  66.07& 64.08 \\
% Instruction&  66.60& 63.33 \\
% Role&  66.82& 63.20\\ \midrule
% Instruction SR (k=1)&  61.69& 71.26\\
% Role SR (k=1)&  61.06& 72.51\\
% Instruction SR (k=2)&  61.36& 71.92\\
% Role SR (k=2)&  61.13& 72.44\\ \midrule
% Instruction IP&  61.93& 70.69\\
% Zero-Shot CoT IP&  61.74& 70.97\\
%  Fewshot IP& 62.27&70.30\\ \midrule
%  SDB Gender& 60.95&71.47\\
%  SDB Race& 62.02&70.03\\
%  SDB Religion& 62.51&69.57\\ \midrule
%  CAFIE& \textbf{59.02}&\textbf{74.72}\\ \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}

% \begin{table}[!htb]
%     \begin{minipage}{.5\linewidth}
%       % \centering
%       \small
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{l|cc}
%     \toprule
% Method&  SS& ICAT \\ \midrule
% Base&  66.07& 64.08 \\
% Instruction&  66.60& 63.33 \\
% Role&  66.82& 63.20\\ \midrule
% Instruction SR (k=1)&  61.69& 71.26\\
% Role SR (k=1)&  61.06& 72.51\\
% Instruction SR (k=2)&  61.36& 71.92\\
% Role SR (k=2)&  61.13& 72.44\\ \midrule
% Instruction IP&  61.93& 70.69\\
% Zero-Shot CoT IP&  61.74& 70.97\\
%  Fewshot IP& 62.27&70.30\\ \midrule
%  SDB Gender& 60.95&71.47\\
%  SDB Race& 62.02&70.03\\
%  SDB Religion& 62.51&69.57\\ \midrule
%  CAFIE& \textbf{59.02}&\textbf{74.72}\\ \bottomrule
%     \end{tabular}
%     }
%     \caption{StereoSet scores comparing prompting strategies with post-hoc debiasing methods on Llama 2.}
%     \end{minipage}%
%     \begin{minipage}{0.5\linewidth}
%       % \centering
%         \resizebox{\linewidth}{!}{
%         \begin{tabular}{l|cc}
%         \toprule
% Method        & SS    & ICAT  \\ \midrule
% Instruction-1 & 66.85 & 60.39 \\
% Instruction-2 & 65.30 & 63.97 \\
% Instruction-3 & 65.49 & 63.31 \\
% Instruction-4 & 65.52 & 63.57 \\ \cdashline{1-3}
%  Average       & 65.79 & 62.81 \\ \midrule
% Role-1        & 63.78 & 66.80 \\
% Role-2        & 63.78 & 66.03 \\
% Role-3        & 64.63 & 64.41 \\
% Role-4        & 63.56 & 66.91 \\ \cdashline{1-3}
%  Average       & \textbf{63.94} & \textbf{66.04} \\ \bottomrule
% \end{tabular}
% }
%     \caption{StereoSet scores upon varying the choice of Instruction and Role Prefixes on Llama 2}
%     \end{minipage}
% \end{table}

\begin{table}[!htb]
    
%     \begin{subtable}{.45\linewidth}
%       \centering
%         \resizebox{\linewidth}{!}{
%         \begin{tabular}{l|cc}
%\toprule
% Method        & SS    & ICAT  \\ \midrule
% Instruction-1 & 66.85 & 60.39 \\
% Instruction-2 & 65.30 & 63.97 \\
% Instruction-3 & 65.49 & 63.31 \\
% Instruction-4 & 65.52 & 63.57 \\ \midrule
%  Average       & 65.79 & 62.81 \\ \midrule
% Role-1        & 63.78 & 66.80 \\
% Role-2        & 63.78 & 66.03 \\
% Role-3        & 64.63 & 64.41 \\
% Role-4        & 63.56 & 66.91 \\ \midrule
%  Average       & \textbf{63.94} & \textbf{66.04} \\ \bottomrule
% \end{tabular}
% }
%     \caption{}
%     \label{prefix_abl}
%     \end{subtable}%
    % \begin{subtable}{.55\linewidth}
      \centering
      \small
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{l|cc}
    \toprule
Method&  SS& ICAT \\ \midrule
Base&  66.07& 64.08 \\
Instruction&  66.60& 63.33 \\
Role&  66.82& 63.20\\ \midrule
Instruction SR (k=1)&  61.69& 71.26\\
Role SR (k=1)&  61.06& 72.51\\ \midrule
% Instruction SR (k=2)&  61.36& 71.92\\
% Role SR (k=2)&  61.13& 72.44\\ \midrule
Instruction IP&  61.93& 70.69\\
Zero-Shot CoT IP&  61.74& 70.97\\
 Fewshot IP& 62.27&70.30\\ \midrule
 SDB Gender& 60.95&71.47\\
 SDB Race& 62.02&70.03\\
 SDB Religion& 62.51&69.57\\ \midrule
 CAFIE& \textbf{59.02}&\textbf{74.72}\\ \bottomrule
    \end{tabular}
    % }
    \caption{Quantitative comparison between post-hoc debiasing methods and prompt-based debiasing strategies.}
    \label{impl_size_abl}
    % \end{subtable}%
\end{table}

==> methodology-simra.tex <==
\section{Methodology}
\label{sec:method}

%\subsection{Our Approach: Introspective Prompting (IP) Framework}

\noindent In this section, we describe the prompting strategies we use to mitigate biases or stereotypes in language model outputs. We structure these approaches into three broad types based on the kind of information provided to the LM. In the first method, \textbf{Prefix Prompting}, we simply direct the model to not be biased while processing the input user text. The second type, \textbf{Self Refinement}, involves a multi-step process where the LM's output, which may be biased, is provided along with the input text to produce fairer results in the subsequent generations. Finally, the third category, \textbf{Introspective Prompting}, is a multi-step process wherein the LM is made to reason about its biased outputs. \\


% As observed by [cite borchers et al] it is not feasible for a single prompt to effectively debias a model's output. We argue that more often than not, the model will be able to eliminate explicit bias, the kind that borders on toxicity or hate speech, but will still exhibit slightly subtler biases. These subtler biases manifest as stereotypical associations made by the model between demographic groups and traits or occupations. 
% In this section, we describe the structure of prompting frameworks we use for fair text generation. \\
% We experiment with three prompting architectures: (i) A simple prefix added to the prompt (1 call to the model) \\
% (ii) A k-step refinement framework that shows the model its previous output as reference (k+1 calls to the model) \\
% (iii) A novel introspective framework that makes the model identify biases present in its own output and uses that as feedback (3 calls to the model). \\


\noindent\textbf{Notations.} Given an input user text $C$ represented as a sequence of tokens ($x_1, \ldots, x_{N}$), and a multi-step or single-step debiasing prompting strategy which modifies $C$ by strategically adding a debiasing prompt $I_{\text{debias}}$, forming $C_{\text{debias}} = \text{concat}(I_{\text{debias}}, C)$. Each of the three prompting strategies differs in $I_{\text{debias}}$ and the steps to get $C_{\text{debias}}$. Let $M$ be a pre-trained language model with a token vocabulary $V$. The model $M$ generates a probability distribution $P_o: V \rightarrow [0,1]$ over the vocabulary for the next token, based on the modified input $C_{\text{debias}}$. Employing a decoding strategy, $P_o$ is used to stochastically sample subsequent tokens ($x_{N+1}, x_{N+2}, \ldots$), resulting in the generation of the output text $S$. Thus, the relationship between the input user text and the output text generated by the model is represented as $M(C_{\text{debias}}, V) = S$.


%Let $M$ be a pre-trained language model with token vocabulary $V$. Given a prompt $C$ represented as a sequence of tokens ($x_1 \ldots x_{N}$), $M$ generates a probability distribution $P_o: V \rightarrow [0,1]$. Subsequently, employing a decoding strategy, $P_o$ is utilized to stochastically sample the next tokens ($x_{N+1}$, $x_{N+1}$ \ldots) and generate the output text $S$. Thus, we have $M(C,V) = S$.


\subsection*{\textsf{Prefix Prompting}: Mitigate by \textit{requesting}}

% In this approach, we prepend a prefix to the input user prompt, and instruct the model to produce unbiased outputs. More specifically, given ${C}$ be a prompt that may introduce biases in the language model output, we prepend it with a debiasing prefix ${I}_{\text{debias}}$ to obtain the final prompt ${C}_{\text{debias}} = \text{concat}({I}_{\text{debias}}, {C}) $.  Our experiments employ two types of prefixes, described next.\\

In this approach, we add a debiasing prefix to the input user text to steer the model towards generating unbiased outputs. %Specifically, let ${C}$ be an input text that may introduce biases in the language model output, we prepend it with a debiasing prefix ${I}_{\text{debias}}$ to obtain the final prompt ${C}_{\text{debias}} = \text{concat}({I}_{\text{debias}}, {C}) $.  Our experiments employ two types of prefixes, described next.\\
Specifically, ${I}_{\text{debias}}$ is an instruction or role-based prefix prompt that is prepended to the input user text ${C}$ that may otherwise introduce biases in the language model output. %The two ${I}_{\text{debias}}$ prompts are: 


% The first prefix we used is a generic instruction.
% \textbf{1. Instruction-Based} \\

\begin{tcolorbox}[colback=gray!10, % Grayscale background color
                  colframe=black, % Frame color
                  sharp corners, % Option for square corners
                  boxsep=5pt, % Padding between text and box
                  left=2pt,right=2pt,top=2pt,bottom=2pt, % Adjust spacing inside the box
                  ]
\textbf{Instruction-Based Prefix Prompt:} \newline The following text is unbiased and does not discriminate against people on the basis of their gender, race, religion, or any other sensitive attribute: [\texttt{INPUT}, $C$]
\end{tcolorbox}
% \textbf{2. Role-Based} \\

\begin{tcolorbox}[colback=gray!10, % Grayscale background color
                  colframe=black, % Frame color
                  sharp corners, % Option for square corners
                  boxsep=5pt, % Padding between text and box
                  left=2pt,right=2pt,top=2pt,bottom=2pt, % Adjust spacing inside the box
                  ]
\textbf{Role-Based Prefix Prompt:} \newline \underline{You are an unbiased person} who does not discriminate against people on the basis of their gender, race, religion, or any other sensitive attribute. [\texttt{INPUT}, $C$] %\\ \newline [Input User Text ($C$)].
\end{tcolorbox}



% \noindent \begin{tikzpicture}
%     \node[draw, rectangle, rounded corners, very thick, text width=0.46\textwidth, align=left] (text) {\fontfamily{cmtt}{\selectfont \small The following text is unbiased and does not discriminate against people on the basis of their gender, race, religion, or any other sensitive attribute:} [\textit{input user text}, $C$]};  
%     \node[above] at (text.north) {Instruction-Based Prefix};
% \end{tikzpicture} \\

% \begin{tikzpicture}
%     \node[draw, rectangle, rounded corners, very thick, text width=0.46\textwidth, align=left]{\fontfamily{cmtt}{\selectfont \small You are an unbiased person who does not discriminate against people on the basis of their gender, race, religion, or any other sensitive attribute.} [\textit{input user text}, $C$]};
%     \node[above] at (text.north) {Role-Based Prefix};
% \end{tikzpicture} 




% Formally, the debiased promp
% t ${C}_{\text{debiased}}$ is given by the concatenation of the source context $C_{\text{source}}$ and the biased instruction ${I}_{\text{debiased}}$:

% \[
% {C}_{\text{debiased}} = C_{\text{source}} \oplus {I}_{\text{debiased}}
% \]
% The objective of introducing ${I}_{\text{debiased}}$ is to guide the language model ${M}$ towards generating unbiased outputs by discouraging the influence of sensitive attributes. This approach aims to modify the output ${C}_{output}$ such that it is less prone to biases associated with the sensitive attributes.
% Hence, we have
% \[
% {M}(C_{\text{source}}, {V}) = {S}_{biased}
% \]
% \[
% {M}(C_{\text{debiased}}, {V}) = {S}_{debiased}
% \]
% \begin{algorithm}
% \caption{Prefix Prompting}
% \label{algorithm:example}
% \begin{algorithmic}
% \State \textbf{Input:} Original Prompt ${C}}$, prefix ${I}$ \\ \newline
% \State \textbf{Output:} Unbiased Text ${S}_{\text{debiased}}$ \\ \newline 
% \State C_{\text{debiased}} \leftarrow {I} \Vert C \\ \newline
% \State {S}_{\text{debiased}} \leftarrow {M}(C_{\text{debiased}}, {V})
% \end{algorithmic}
% \label{alg-1}
% \end{algorithm}
% \begin{figure} 
%     \centering
%     \includegraphics[width=0.5\textwidth]{latex/Images/p1.pdf}
%     \caption{List of Single-Step Prompts}
%     \label{fig:Prefixes-1}
% \end{figure}
\subsection*{Self Refinement (SR): Mitigate by \textit{Iterative Refining}}
% We observed that the outputs generated with a simple single-step prefix prompting still possessed a substantial bias. Thus, we extend it to a k-step approach where our objective is to obtain more refined outputs by asking the model to refer to its previous step outputs for carrying out subsequent generations. We describe this strategy for k=2 below, and provide its generic formulation in Algorithm 1. \\
% {\color{red} SEGUE }
% In this framework, the initial output serves as a reference text, which is combined with a new instruction to prompt subsequent iterations. \\

In this $k$-step self-refinement approach, the language model is invoked to critically evaluate and reduce biases in its prior outputs through iterative adjustment. This allows the model to correct for complex biases step-by-step that may have been missed in a single iteration. Specifically, ${I}_{\text{debias}}$ is an instruction or role-based SR prompt, ${I}_{\text{SR}}$, that takes the \textit{previous output} of the model for $k$ steps. 

%until the stopping criterion $k$. 
%which has been already prompted to correct for bias 

\begin{tcolorbox}[colback=gray!10, % Grayscale background color
                  colframe=black, % Frame color
                  sharp corners, % Option for square corners
                  boxsep=5pt, % Padding between text and box
                  left=2pt,right=2pt,top=2pt,bottom=2pt, % Adjust spacing inside the box
                  ]
\textbf{Instruction-Based SR Prompt:} \newline Here is a text you generated: [\texttt{OUTPUT}]\\ Now refer to this text and generate some text that is unbiased and does not discriminate against people on the basis of their gender, race, religion, or any other sensitive attribute.  [\texttt{INPUT}, $C$]
\end{tcolorbox}
% \textbf{2. Role-Based} \\

\begin{tcolorbox}[colback=gray!10, % Grayscale background color
                  colframe=black, % Frame color
                  sharp corners, % Option for square corners
                  boxsep=5pt, % Padding between text and box
                  left=2pt,right=2pt,top=2pt,bottom=2pt, % Adjust spacing inside the box
                  ]
\textbf{Role-Based SR Prompt:} \newline Here is a text you generated: [\texttt{OUTPUT}]\\  Now refer to this text considering that \underline{you are an unbiased person} who does not discriminate against people on the basis of their gender, race, religion, or any other sensitive attribute.  [\texttt{INPUT}, $C$] %\\ \newline [Input User Text ($C$)].
\end{tcolorbox}


\noindent Next, we describe the steps of Self Refinement as formulated in Algorithm 1. 

\noindent \textbf{Step 1} -- Given the input user text $C$, we first perform the Prefix Prompting strategy to obtain output $S_0$, which is the reference text for the LM's subsequent generation. \\
\textbf{Step 2a} -- We then combine $S_0$ with self refinement prompt to obtain the output of the next step ${C}_{\text{SR}} = \text{concat}({I}_{\text{SR}}, S_0, C)$. \\
\textbf{Step 2b} -- With this prompt, we query the language model and generate an output $S_1$. \\
The \textbf{Steps 2a} and \textbf{2b} are repeated till the stopping criterion, i.e, the number of iterations $k$. 

\begin{algorithm}
\caption{Self-Refinement Prompting}
\begin{algorithmic}[1]
\REQUIRE Input User Text $C$, Debiasing Prefix $I_{\text{SR}}$, Number of Iterations $k$
\ENSURE Unbiased Text $S_{\text{debiased}}$
\\ \hrulefill
\STATE \textbf{Step 1: Prefix Prompting}
\STATE $C_{\text{debias}} = \text{concat}(I_{\text{SR}}, C)$
\STATE $S_0 \leftarrow M(C_{\text{debias}}, V)$
\STATE \textbf{Step 2: Iterative Self-Refinement}
\FOR{$i = 1$ \TO $k$}
    \STATE \textbf{Step 2a:} $C_{\text{SR}} \leftarrow \text{concat}(I_{\text{SR}}, S_{i-1}, C)$ 
    \STATE \textbf{Step 2b:} $S_i \leftarrow M(C_{\text{SR}}, V)$ 
\ENDFOR
\STATE $S_{\text{debiased}} \leftarrow S_k$
\end{algorithmic}
\end{algorithm}



% \begin{algorithm}
% \caption{Self-Refinement Prompting}
% % \label{alg: self-refinement}
% \begin{algorithmic}[1]
% \REQUIRE Input User Text $C$, Debiasing Prefix ${I}_{\text{SR}}$, Number of Iterations $k$
% \ENSURE Unbiased Text ${S}_{\text{debiased}}$\\
% \hline
% \textbf{Step I}: Prefix Prompting
% \STATE $C_{\text{debias}} = \text{concat}(I_{\text{debias_prefix}}, C)$ // 
% \STATE $S_0 \leftarrow M(C_{debias}, V)$ // 
% \FOR{$i \in [1, k]$}
%     \STATE $C_{\text{SR}} \leftarrow concat({I}_{\text{SR}}, S_{i-1}, C)$
%     \STATE $S_i \leftarrow M(C_{\text{SR}}, V)$
% \ENDFOR
% \STATE ${S}_{\text{debiased}} \leftarrow S_k$
% \end{algorithmic}
% \label{alg-2}
% \end{algorithm}

% \begin{algorithm}
% \caption{Self-Refinement Prompting}
% \begin{algorithmic}[1]
% \REQUIRE Input User Text $C$, Debiasing Prefix $I_{\text{SR}}$, Number of Iterations $k$
% \ENSURE Unbiased Text $S_{\text{debiased}}$
% \\ \hrulefill \\
% \textbf{Step 1: Prefix Prompting}
% \STATE $C_{\text{debias}} = \text{concat}(I_{\text{SR}}, C)$ 
% \STATE $S_0 \leftarrow M(C_{\text{debias}}, V)$ \\
% \vspace{2mm}
% %\textbf{Step 2: Iterative Self-Refinement}
% \FOR{$i = 1$ \TO $k$}
%     \textbf{Step 2:} \STATE $C_{\text{SR}} \leftarrow \text{concat}(I_{\text{SR}}, S_{i-1}, C)$ 
%     \\
%     \textbf{Step 3:} \STATE $S_i \leftarrow M(C_{\text{SR}}, V)$ 
% \ENDFOR
% \STATE $S_{\text{debiased}} \leftarrow S_k$ 
% \end{algorithmic}
% \end{algorithm}



% \begin{tikzpicture}
%     \node[draw, rectangle, rounded corners, very thick, text width=0.46\textwidth, align=left] (text) {\fontfamily{cmtt}\selectfont \small Here is a text you generated: [OUTPUT]\\ Now refer to this text and generate some text that is unbiased and does not discriminate against people on the basis of their gender, race, religion, or any other sensitive attribute.};  
%     \node[above] at (text.north) {Instruction-Based SR Prompt};
% \end{tikzpicture}
% \begin{tikzpicture}
%     \node[draw, rectangle, rounded corners, very thick, text width=0.46\textwidth, align=left] (text) {\fontfamily{cmtt}\selectfont \small Here is a text you generated: [OUTPUT]\\  Now refer to this text considering that you are an unbiased person who does not discriminate against people on the basis of their gender, race, religion, or any other sensitive attribute.};  
%     \node[above] at (text.north) {Role-Based SR Prompt};
%     % \textcolor{red}{Fix }
% \end{tikzpicture}

\subsection*{Introspective Prompting (IP): Mitigate by \textit{Reasoning}}

%\noindent\textbf{Implication.} The notion of `implication' here refers to the underlying biases or stereotypes that may be present in the generated output $S$. Identifying these implications is crucial for understanding and mitigating unwanted biases in language models. For example, for the input query in figure \ref{fig:Implication}, the implication is that `women are less qualified than men'. 



% {\color{red} TRIM}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{latex/Implicative_introspection.jpg}
%     \caption{Flow diagram of the Dual-Step Implication Prompting Framework}
%     \label{fig:Implication}
% \end{figure}

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{latex/Implicative_introspection.jpg}
%     \caption{Flow diagram of the Introspective Prompting Framework}
%     \label{fig:Implication}
% \end{figure}

% To achieve this, we first 
% Noting that even k-step prefix prompting reached a plateau in performance after k=3, we developed a framework to provide explicit feedback to the LM about its output. We theorize that similar to how biases seep into LLMs through training data, knowledge and understanding of social biases also make their way into these latent spaces. Thus, probing a model about the potential implications of its generation provided us with accurate feedback about bias. These implications were then used to generate the final unbiased response. \\
% Concretely, this framework is divided into three steps (see Algorithm \ref{alg-3} and Figure \ref{fig:Implication}).\\


In the previous approach, it can be challenging for the LM to simply refer to its own biased outputs for generating fair text. Thus, we hypothesize that a better way would be that alongside its self-generated biased text, the LM also refers to a reasoning or implication of why that output is biased. Given that we cannot hard-code implications corresponding to every possible model output, we propose to generate the such implications on-the-fly using the LM itself. More concretely, we divide this framework into three steps (see Algorithm \ref{alg-3}), described next.\\
\noindent\textbf{Step I} -- The first input to the LM is simply the user prompt $C$ that generates an output $S$ which might be biased.\\
\noindent\textbf{Step II} -- The next input to the LM is $C_{impl}$, a prompt made using the initial output $S$ concatenated with an instruction $I_{impl}$. This instruction asks the model to generate the \textit{Implication} $S_{Impl}$ of the output $S$. The goal of this step is to make the model identify any biases or stereotypes present in the initial output. We employ three different types of $I_{impl}$ for our experiments. \\  
\begin{tcolorbox}[colback=gray!10, % Grayscale background color
                  colframe=black, % Frame color
                  sharp corners, % Option for square corners
                  boxsep=5pt, % Padding between text and box
                  left=2pt,right=2pt,top=2pt,bottom=2pt, % Adjust spacing inside the box
                  ]
\textbf{Instruction-Based $C_{Impl}$:} \newline Here is a text: [\texttt{OUTPUT}] \\ Generate the implication of the given text:
\end{tcolorbox}

\begin{tcolorbox}[colback=gray!10, % Grayscale background color
                  colframe=black, % Frame color
                  sharp corners, % Option for square corners
                  boxsep=5pt, % Padding between text and box
                  left=2pt,right=2pt,top=2pt,bottom=2pt, % Adjust spacing inside the box
                  ]
\textbf{Zero-Shot CoT-Based $C_{Impl}$:} \newline Here is a text: [\texttt{OUTPUT}] \\ Thinking step by step, generate the implication of the given text:
\end{tcolorbox}

\begin{tcolorbox}[colback=gray!10, % Grayscale background color
                  colframe=black, % Frame color
                  sharp corners, % Option for square corners
                  boxsep=5pt, % Padding between text and box
                  left=2pt,right=2pt,top=2pt,bottom=2pt, % Adjust spacing inside the box
                  ]
\textbf{Fewshot-Based $C_{Impl}$:} \newline For each text, generate the implication which shows the stereotype present in the text. \newline
[Text 1]: We shouldn't lower our standards just to hire more women. \newline
[Implication 1]: This text implies that woman are less qualified than men. \newline
. \newline
. \newline
[Text 4]: [\texttt{OUTPUT}]\newline
[Implication 4]: 
\end{tcolorbox}


\noindent\textbf{Step III} -- The final prompt $C_{IP}$ combines the model's initial biased output $S$, the generated implication $S_{Impl}$, and an instruction $I_{IP}$. This prompt contextualizes the original output for the model with the stereotypes and biases present within it and directs the model to generate an unbiased text without those biases.\\\\
\begin{tcolorbox}[colback=gray!10, % Grayscale background color
                  colframe=black, % Frame color
                  sharp corners, % Option for square corners
                  boxsep=5pt, % Padding between text and box
                  left=2pt,right=2pt,top=2pt,bottom=2pt, % Adjust spacing inside the box
                  ]
\textbf{Zero-Shot CoT-Based $C_{IP}$:} \newline You are an unbiased person who does not discriminate against people on the basis of their gender, race, religion, or any other sensitive attribute. \newline
Here is a sentence you generated: [\texttt{OUTPUT}]\newline
Here is the implication that indicates the bias present in the text: [\texttt{IMPLICATION}]\newline
Now, considering the implication and referring to the original sentence, generate an unbiased text that does not discriminate against people on the basis of their gender, race, religion, or any other sensitive attribute: [\texttt{INPUT}, $C$]
\end{tcolorbox}

\begin{algorithm}
\caption{Introspective Prompting}
% \label{algorithm:introspective_prompting}
\begin{algorithmic}[1]
\REQUIRE Original Prompt $C$, instructions $I_{\text{impl}}$ and $I_{\text{IP}}$
\ENSURE Unbiased Text $S_{\text{debiased}}$
\STATE $S \leftarrow M(C, V)$
\STATE $C_{\text{Impl}} \leftarrow concat(S,I_{\text{Impl}})$
\STATE ${S}_{\text{Impl}} \leftarrow {M}(C_{\text{Impl}}, {V})$
\STATE $C_{\text{IP}} \leftarrow concat({S}, {S}_{\text{Impl}},I_{\text{IP}}, C)$
\STATE ${S}_{\text{debiased}} \leftarrow {M}(C_{\text{IP}}, {V})$
\end{algorithmic}
\label{alg-3}
\end{algorithm}

==> posthoc_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[!ht]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
Method                   & \multicolumn{1}{c}{SS}   & \multicolumn{1}{c}{ICAT} & \multicolumn{1}{c}{TruthfulQA}  & \multicolumn{1}{c}{BoolQ} \\ \midrule
GPTJ (6B)                & $66.07$                  & $64.08$                  & $48.96$                         & $40.61$   \\
Instruction              & $66.60$                  & $63.33$                  & $42.72$                         & $43.76$   \\
Role                     & $66.82$                  & $63.20$                  & $45.78$                         & $39.95$   \\ \midrule
Instruction SR (k=1)     & $61.69$                  & $71.26$                  & $43.21$                         & $40.65$   \\
Role SR (k=1)            & $61.06$                  & $72.51$                  & $41.13$                         & $43.18$   \\
Instruction SR (k=2)     & $61.36$                  & $71.92$                  & $44.92$                         & $41.74$   \\
Role SR (k=2)            & $61.13$                  & $72.44$                  & $41.98$                         & $41.88$   \\ \midrule
Instruction IP           & $61.93$                  & $70.69$                  & $52.63$                         & $41.49$   \\
Zero-Shot CoT IP         & $61.74$                  & $70.97$                  & \textbf{$54.35$}                & $41.52$   \\
Fewshot IP               & $62.27$                  & $70.30$                  & $50.12$                         & $41.43$   \\ \midrule
SelfDebias Gender        & $60.95$                  & $71.47$                  & $34.52$                         & $61.10$   \\
SelfDebias Race          & $62.02$                  & $70.03$                  & $34.64$                         & \textbf{$61.13$}   \\
SelfDebias Religion      & $62.51$                  & $69.57$                  & $34.52$                         & $61.10$   \\ \midrule
SentenceDebias Gender    & $62.73$                  & $69.44$                  & $49.94$                         & $40.89$   \\ 
SentenceDebias Race      & $62.35$                  & $69.73$                  & $53.86$                         & $41.34$  \\ 
SentenceDebias Religion  & $62.91$                  & $69.12$                  & $50.06$                         & $40.04$  \\ \midrule
CAFIE                    & $\textbf{59.02}$         & $\textbf{74.72}$         & $36.72$                         & $17.43$   \\ \bottomrule
\end{tabular}
}
\caption{Comparison against post-hoc and white-box debiasing methods on StereoSet, TruthfulQA, and BoolQ. \label{tab:cafie}}

\end{table}
